Efficient Query Repair for Aggregate Constraints

In many real-world scenarios, query results must satisfy domain-specific constraints. For instance, a minimum percentage of interview candidates selected based on their qualifications should be female. These requirements can be expressed as constraints over an arithmetic combination of aggregates evaluated on the result of the query. In this work, we study how to repair a query to fulfill such constraints by modifying the filter predicates of the query. We introduce a novel query repair technique that leverages bounds on sets of candidate solutions and interval arithmetic to efficiently prune the search space. We demonstrate experimentally, that our technique significantly outperforms baselines that consider a single candidate at a time.

==> Sections/Section2.tex <==
\section{Example Use Cases}\label{sec:usecases} %Copied from TapP paper

%\BGI{I think one problem we have with the current structure is that we already walk through a relatively detailed fairness example in the intro making this section partially redundant. One option could be to merge this example intro and align it with Figure 1.}

% We describe two use cases to highlight the need for repairing user queries to fulfill aggregate constraints on the query's result.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Company Product Management}\label{subsec:generalUse}

%Consider a supply and demand scenario over the TPC-H Benchmark schema~\cite{tpc-hLink}.
A retail company aims to monitor product performance by retrieving information about the parts of type “Large Brushed” with a size greater than 10 that are supplied by suppliers located in Europe.\BG{This sounds different from the paragraph after the query which talks about product selection for stock management. We need to align these two.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The company uses the following query to retrieve this information:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \mypar{The Query}
\begin{lstlisting}
@\small\upshape\bf\ttfamily{Q2}@: SELECT *
    FROM part, supplier, partsupp, nation, region
    WHERE p_partkey = ps_partkey AND
        s_suppkey = ps_suppkey AND p_size >= 10
        AND s_nationkey = n_nationkey
        AND n_regionkey = r_regionkey
        AND p_type = 'LARGE BRUSHED'
        AND r_name = 'EUROPE'
\end{lstlisting}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%This query is hardcoded in the company's inventory management system, which is maintained by an external vendor. The system is designed to automatically retrieve all relevant product and supplier details, ensuring uniformity in reporting across all company branches. As a result, the manager cannot modify the query logic directly.

The company, however, has set an aggregate constraint to manage its product selection and ensure effective inventory planning. They want to avoid overstocking under-performing products that contribute less to revenue.\BG{This is not reflected in the constraint!}
The constraint requires that products from UK only contribute 10\% to 30\% of the total revenue of the result set in order to minimize supply chain disruptions. Formally, the constraint is defined as follows:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-2mm}
% \[
% 0.3 \leq \frac{\sum \text{Revenue}_{\text{Selected Products}}}{\sum \text{Revenue}_{\text{All Products}}} \leq 0.5
% \]
\[
0.1 \leq \frac{\sum \text{Revenue}_{\text{ProductsSelectedFromUK}}}{\sum \text{Revenue}_{\text{Selected Products}}} \leq 0.3
\]
% Where:

% $\text{Revenue}_{\text{Selected Products}} = \sum (l\_extendedprice \times (1 - l\_discount))$ and $\sum \text{Revenue}_{\text{All Products}} = \sum (l\_extendedprice \times (1 - l\_discount))$ for all products.


Prior work on query repair ~\cite{AlbarrakS17} only supports constraints on a single aggregation result while the constraint shown above is an arithmetic combination of aggregation results as supported in our framework. % , e.g., simplistic average using a single attribute from the dataset.
% In this case, we have a aggregation over multiple attributes.


%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "../main"
%%% End:


==> Sections/Section6_old.tex <==
\section{Experiments} \label{sec:expermint}
% We conducted an empirical evaluation of our proposed techniques to demonstrate their performance. The evaluation includes a detailed description of the experimental setup and a quantitative analysis of our algorithm's efficiency. This analysis encompasses various datasets, queries, and arithmetic constraints.


We evaluate the performance
% and effectiveness
of our algorithms using real-world and TPC-H benchmark datasets. % various queries, and numerous arithmetic constraints.
% The performance is based on three factors: (i) runtime, (ii) the total number of constraints evaluated (NCE), and (iii) the total number of cluster accessed (NCA).
% Each performance evaluation was repeated five times and we report the median runtime as the variance is low ($\sim 3\%$).
% % The experiment begins by comparing our proposed techniques to the brute-force approach in~\Cref{subsec: cpmare with brute force}, illustrating that the brute-force approach is not a viable competitor due to its inefficiency.
% % We then evaluate
We start by comparing
the baseline \gls{algff} technique (\Cref{subsec: baseline}) against our \gls{algrp} algorithm (\Cref{sec:Range})  in~\Cref{subsec: compare proposed techniques}. %Additionally,
We then investigate the impact of several  factors, such as dataset size and how similar the top-k repairs are to the user query,  on performance in~\Cref{subsec: invistigation}. Finally, we compare our approach
with \emph{\gls{erica}}~\cite{LM23}, which only supports cardinality constraints over groups in the query output by generating all minimal refinements, in~\Cref{subsec: compare with related work}. Note that \gls{erica} uses a different optimization criterion than we do: as in skyline queries, \emph{minimal refinements} in \gls{erica} are repairs that where none of the predicates can be further refined and still yield a repair. In contrast we compare repairs based on a distance metric. We will explain in \Cref{subsec: compare with related work} how we achieve a fair comparison.
% We use the following key metrics to compare the performance:
% \begin{itemize}
%     \item \textbf{Execution Time (s):} The duration required for the query repair techniques to complete (Brute force, \gls{algff} and \gls{algrp} Query Repair techniques).
%     \item \textbf{Number of Candidate Solutions Checked:} The total number of constraints evaluated for all possible repairs executing by the repair technique.
%     \item \textbf{Number of Clusters Accessed:} The total number of accessed clusters in the cluster tree.
% \end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experimental Setup}
\label{sec:setup}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Datasets}
We choose two real-world datasets of size of 500K, \emph{\gls{dsacs}}~\cite{FriedlerSVCHR19} and \emph{\gls{dshealth}}~\cite{grafberger2021mlinspect}, that are commonly used to evaluate fairness.
% use case.
% with dataset size of 500K.
% as default.
We also utilize a standard benchmark, \emph{\gls{tpch}}~\cite{tpc-hLink},
% for measuring the performance and effectiveness of
to varying dataset size
% as a common benchmark which contains 61 attributes in total. We varied dataset size
from 25K to 500K.
We converted categorical columns into numerical data as the algorithms are designed for numerical data.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Queries}
\Cref{tab:queries} shows the queries used in our experiments. For \gls{dshealth}, we use queries $Q_1$ and $Q_2$ from~\cite{LM23} and a new query $Q_3$.
For \gls{dsacs}, we use $Q_4$ from~\cite{LM23} and new queries $Q_5$ and $Q_6$.
% However, since our techniques are designed to handle only numerical data, we converted the categorical attributes from the original data into numerical values. Consequently, we updated queries Q1 and Q4 to accommodate these changes, ensuring they align with the requirements of our approach.
%For TPC-H,
We generated %two SPJ query
$Q_7$ with 3 predicates inspired by \gls{tpch}'s $Q_2$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Constraints}
%
For \gls{dshealth} and \gls{dsacs}, we enforce the \gls{SPD} between two demographic groups to be within a certain bound.
\Cref{tab:constraints} shows the details of the constraints used. In some experiments, we vary the bounds
$B_l$ and $B_u$. For a constraint $\propconstr_i$ we use $\propconstr_i^{d=p}$ to denote a variant of $\propconstr_i$ where the bounds have been set such that the top-k repairs are within the first p\% of the repair candidates ordered by distance to the user query. In other words, an algorithm that explores the individual repair candidates in this order would have to explore the first p\% of the candidate search space to find the top-k repairs.
% the constraints are
% $\propconstr_{1}$ and $\propconstr_{2}$ are the constraints for the \gls{dshealth} dataset with various bounds between 0.2 and 0.6.
% Similarly, $\propconstr_{3}$ and $\propconstr_{4}$ are the constraints for the ACSIncome dataset with multiple bounds between 0.2 and 0.5.
For the detailed settings see~\cite{AG25techrepo}.
For \gls{dsacs}, we determine the groups for \gls{SPD} based on gender and race. For \gls{dshealth}, we determine demographic groups based on race and age group.
% shown in \texttt{Bounds} of the table. %[lower bound,upper bound].
For \gls{tpch}, we enforce the constraint $\propconstr_{5}$ to avoid overstocking under-performing products that
contribute less to revenue. % from the use case in \Cref{subsec:generalUse} to be larger than or equal to a specific value
This ensures that UK products contribute only a specific percentage of total revenue, minimizing supply chain disruptions.
We use $\propconstrset$ to denote a set of \glspl{AC}.
$\propconstrset_{6}$ through $\propconstrset_{8}$ are sets of cardinality constraints for comparison with \gls{erica}. While we have presented our repair methods for single \glspl{AC}, the methods can be trivially extended to find repairs for a set of constraints, i.e., the repair fulfills $\bigwedge_{\propconstr \in \propconstrset} \propconstr$. For \gls{algrp} (\Cref{alg:range_filtering}), it is sufficient to replace the condition in Line \ref{algline:acevalall} with $\bigwedge_{\propconstr \in \propconstrset} \acrangeevalall(\propconstr, \clusterset_{full}, \clusterset_{partial})$ and the condition in Line \ref{algline:acevalexists} with $\bigwedge_{\propconstr \in \propconstrset} \acrangeevalexists(\propconstr, \clusterset_{full}, \clusterset_{partial})$.
% \SLI{Why do we have these many different bounds to test?}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \mypar{Number of Candidate Repairs}
% The number of candidate repairs is calculated as the product of the unique possible values for all predicates. For \gls{dsacs} dataset, this number ranges from approximately 14K to 18K. In \gls{dshealth} dataset, it varies between approximately 10K and 22K. For TPCH queries, the number of possible repair candidates is approximately 38K.
 %need to fix for TPCH

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Parameters}
% \SLI{@Seokki: confirm whether the clustering tree structure is clearly explained in previous sections.}
There are three key tuning parameters that could impact the performance of our methods.
Recall that we use a kd-tree to perform the clustering described in Section \ref{subsec:clustering}.
% in the following manner:
We consider two tuning parameters for the tree:
\begin{itemize}[leftmargin=1em]
\item \textbf{Branching Factor}: Each node has \branchfactor children.
% in this work we allow
% each cluster is split into multiple branches.
% (controlled by a user-defined branches parameter).

\item \textbf{Bucket Size}:
% To optimize the storage and traversal, a bucket size
  Parameter \bucketsize
% a user-defined Bucket Size parameter)
determines the minimum number of tuples in a cluster. We do not split nodes with less than or equal to $\bucketsize$ tuples. When one of our algorithms reaches such a leaf node we just evaluate computations on each tuple in the cluster, e.g., to determine which tuples fulfill a condition. % stops splitting and assigns the points to individual leaf clusters.

% \item \textbf{Clustering Tree Structure}: Each cluster in the tree contains metadata for further analysis: the level of the cluster in the tree, cluster id which is a unique identifier for each cluster, parent's cluster and level which are reference to the parent cluster and level for hierarchical tracing and the set of points contained in the cluster.
\end{itemize}
% \AC{Merge the paragraph below and the information above.}
% (i) Bucket size, which defines the maximum number of points a cluster in the clustering tree can contain;
% (ii) Branching factor, which specifies the number of branches generated at each node of the clustering tree, as explained in~\Cref{subsec:clustering};
% In all experiments, we use a default bucket size of 15 and a branching factor of 5.
%
% (iii)
We also control $k$, the number of repairs returned by our methods. % umber of repairs to be generated by our techniques.
% In all experiments, we use a default top 7.
The default setting for these parameters is as follows: $\branchfactor = 5$, $k=7$, and $\bucketsize = 15$. The default dataset size is 50K tuples.


% \mypar{Platform}
All algorithms were implemented in Python, and the experiments were conducted on a machine with 2 x 3.3Ghz AMD Opteron CPUs (12 cores) and 128GB RAM.
Each experiment was repeated five times and report the median runtime as the variance is low ($\sim 3\%$).

% \SAI{Boris, could you please add information about the server as I am not sure about it}
% \SLI{Place the ligeti configuration. Please feel free to modify it.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \mypar{Compared Algorithms}
% \begin{itemize}
%     \item \textbf{Brute Force technique (BF):} it enumerates and tests all possible repairs by filtering data by testing all data points.
%     \item \textbf{Fully Filtering Query Repair (\gls{algff}):} described in section \ref{subsec: baseline}. %is a hierarchical method designed to identify clusters where all data points satisfy a possible repair condition. It leverages a top-down traversal strategy to filter clusters based on their materialized bounds (minimum and maximum values) \ref{subsec: baseline}.
%     \item \textbf{Range-Based Pruning Query Repair (\gls{algrp}):} described in section \ref{subsec: optimized gorithm}. %it evaluates constraints over a search space by dividing possible repairs into ranges. It leverages materialized statistical bounds and range division to focus on promising candidate solutions, avoiding exhaustive testing of all possible repairs, as baseline \ref{subsec: optimized gorithm}.
% \end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% To ensure the reliability of our results, we performed \textbf{five repetitions for each experiment} and calculated the \textbf{variance}. Specifically, for each experiment, we computed the \textbf{variance and average runtime}, then determined the \textbf{relative variance} as:
% $\frac{\text{variance}}{\text{average}} \times 100$.
% %
% Across all experiments, the maximum observed relative variance was \textbf{only 3\%}, indicating a high level of consistency in our measurements. Given this low variability, we present a \textbf{single representative runtime} for each experiment in our results.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
    % \centering
    % \vspace{-7mm}
    \caption{Queries for Experimentation}
    \vspace{-2mm}
    \adjustbox{max width=\columnwidth}{
    \begin{tabular}{|c|l|}
    \hline
         % \textbf{ID} & \hspace{45mm}\textbf{Query} \\
         % \hline
         \multicolumn{2}{|l|}{
% \begin{lstlisting}
\lstinline{SELECT * FROM Healthcare}
% \end{lstlisting}
         } \\
         \cline{1-2}
         $Q_1$ &
\begin{lstlisting}
WHERE income >= 200K AND num-children >= 3
      AND county <= 3
\end{lstlisting} \\ \cline{1-2}
  $Q_2$ &
  % \lstset{aboveskip=0pt, belowskip=0pt}
  \begin{lstlisting}
WHERE income <= 100K AND complications >= 5
      AND num-children >= 4
\end{lstlisting} \\
\cline{1-2}
  $Q_3$ &
  % \lstset{aboveskip=0pt, belowskip=0pt}
\begin{lstlisting}
WHERE income >= 300K AND complications >= 5
      AND county == 1
\end{lstlisting} \\ \hline \hline
\multicolumn{2}{|l|}{
% \begin{lstlisting}
\lstinline{SELECT * FROM ACSIncome}
% \end{lstlisting}
         } \\
         \cline{1-2}
  $Q_4$ &
  % \lstset{aboveskip=0pt, belowskip=0pt}
  \begin{lstlisting}
WHERE working_hours >= 40 AND Educational_attainment >= 19
      AND Class_of_worker >= 3
\end{lstlisting} \\ \cline{1-2}
  $Q_5$ &
  % \lstset{aboveskip=0pt, belowskip=0pt}
  \begin{lstlisting}
WHERE working_hours <= 40 AND Educational_attainment <= 19
      AND Class_of_worker <= 4
\end{lstlisting}  \\ \cline{1-2}
  $Q_6$ &
  % \lstset{aboveskip=0pt, belowskip=0pt}
  \begin{lstlisting}
WHERE Age >= 35  AND Class_of_worker >= 2
      AND Educational_attainment <= 15
\end{lstlisting} \\ \hline \hline
% \multicolumn{2}{|l|}{
% % \begin{lstlisting}
% \lstinline{SELECT * FROM part, supplier, partsupp, nation, region}
% % \end{lstlisting}
%          } \\
%          \cline{1-2}
$Q_7$ &
% \lstset{aboveskip=0pt, belowskip=0pt}
\begin{lstlisting}
SELECT * FROM part, supplier, partsupp, nation, region
WHERE p_partkey = ps_partkey AND s_suppkey = ps_suppkey
AND s_nationkey = n_nationkey AND n_regionkey=r_regionkey
AND p_size >= 10 AND p_type in ('LARGE BRUSHED')
AND r_name in ('EUROPE')
\end{lstlisting} \\  \hline
    \end{tabular}
    }
    \label{tab:queries}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t] % Use table* to span both columns
    \centering %\small
    % \vspace{-7mm}
    \caption{Constraints for Experimentation}
    \vspace{-2mm}
    \begin{tabular}{|p{0.2cm}|p{7.6cm}|
    % |p{2cm}|p{8.5cm}|
    % p{6cm}|p{1.2cm}|
    }
    \hline
    \textbf{ID} & \hspace{30mm}\textbf{Constraint}
    % & \textbf{Bounds}
    \\ \hline
    % \\[-3.3mm]
    $\propconstr_{1}$ &
    $ \frac{\f{count}(\text{race} = 1 \land \text{label} = 1)}{\f{count}(\text{race} = 1)} - \frac{\f{count}(\text{race} = 2 \land \text{label} = 1)}{\f{count}(\text{race} = 2)} \in [B_l,B_u]$
    % &
    % $B_1$:[0.44, 0.5], $B_2$:[0.25, 0.5], $B_3$:[0.42, 0.5], $B_4$:[0.35, 0.5], $B_5$:[0.5, 0.6], $B_6$:[0.23, 0.25], $B_7$:[0.25, 0.4], $B_8$:[0.34, 0.39], $B_9$:[0.2, 0.25], $B_{10}$:[0.3, 0.5], $B_{11}$: [0.31, 0.36], $B_{12}$: [0.2, 0.5]
    \\ [1mm]
    \hline
    % \\[-3.3mm]
    $\propconstr_{2}$ &
    {\small $ \frac{\f{count}(\text{ageGroup} = 1 \land \text{label} = 1)}{\f{count}(\text{ageGroup} = 1)} - \frac{\f{count}(\text{ageGroup} = 2 \land \text{label} = 1)}{\f{count}(\text{ageGroup} = 2)} \in [B_l,B_u]$}
    % & $B_1$:[0.44, 0.5], $B_2$:[0.25, 0.5], $B_3$:[0.42, 0.5], $B_4$:[0.35, 0.5], $B_5$:[0.5, 0.6]
    \\ [1mm]
    \hline
    % \\[-3.3mm]
    $\propconstr_{3}$ &
    $ \frac{\f{count}(\text{sex} = 1 \land \text{PINCP} \geq 20k)}{\f{count}(\text{sex} = 1)} - \frac{\f{count}(\text{sex} = 2 \land \text{PINCP} \geq 20k)}{\f{count}(\text{sex} = 2)} \in [B_l,B_u]$
    % &  $B_1$:[0.34, 0.39], $B_2$:[0.3, 0.5], $B_3$:[0.44, 0.5], $B_4$:[0.25, 0.5], $B_5$:[0.2, 0.25], $B_6$:[0.15, 0.4], $B_7$:[0.23, 0.25], $B_8$:[0.22, 0.4], $B_9$:[0.34, 0.36], $B_{10}$:[0.34, 0.35], $B_{11}$:[0.35, 0.36], $B_{12}$:[0.39, 0.4], $B_{13}$:[0.42, 0.44]
    \\ [1mm]
    \hline
    % \\[-3.5mm]
    $\propconstr_{4}$ &
    {\small $ \frac{\f{count}(\text{race} = 1 \land \text{PINCP} \geq 15k)}{\f{count}(\text{race} = 1)} - \frac{\f{count}(\text{race} = 2 \land \text{PINCP} \geq 15k)}{\f{count}(\text{race} = 2)} \in [B_l,B_u]$}
    % & $B_1$:[0.34, 0.39], $B_2$:[0.3, 0.5], $B_3$:[0.44, 0.5], $B_4$:[0.25, 0.5], $B_5$:[0.2, 0.25], $B_6$:[0.37, 0.39], $B_7$:[0.38, 0.39], $B_8$:[0.34, 0.35], $B_9$:[0.34, 0.39], $B_{10}$:[0.3, 0.5], $B_{11}$:[0.23, 0.25], $B_{12}$:[0.34, 0.36], $B_{13}$:[0.3, 0.33], $B_{14}$:[0.32, 0.35]
    \\ [1mm]
    \hline
    % \\[-3.5mm]
    $\propconstr_{5}$ &
    $ \frac{\sum \text{Revenue}_{\text{ProductsSelectedFromUK}}}{\sum \text{Revenue}_{\text{Selected Products}}} \in [B_l,B_u]$
    % & $B_1$: 0.0014, $B_2$: 0.0025, $B_3$: 0.005, $B_4$: 0.01, $B_5$: 0.026
    \\ [1mm]
    \hline
     $\propconstrset_{6}$ &
                            $\propconstr_{61} \defas \f{count}(\text{race}= \text{race1} )  \leq B_{u_1}$ \\
      &$\propconstr_{62} \defas  \f{count}(\text{age}= \text{group1})  \leq B_{u_2}$
    % & 300, 170
      \\
    \hline
     $\propconstrset_{7}$ &
                            $\propconstr_{71} \defas \f{count}(\text{race}= \text{race1})  \leq B_{u_1}$\\
      &$\propconstr_{72} \defas \f{count}(\text{age}= \text{group1})  \leq B_{u_2}$ \\
    & $\propconstr_{73} \defas  \f{count}(\text{age}= \text{group3})  \leq B_{u_3}$
    % & 300, 170,250
    \\
    \hline
    $\propconstrset_{8}$ &
{\small $\propconstr_{81} \defas \f{count}(\text{Sex}= \text{Female})  \leq B_{u_1}$}\\
&{\small $\propconstr_{82} \defas \f{count}(\text{Race}= \text{Black})  \leq B_{u_2}$ } \\
& {\small $\propconstr_{83} \defas \f{count}(\text{Marital}= \text{Divorced})  \leq B_{u_3}$ }
% &
% $\text{B1}=30, 150, 10, \quad \text{B2} = 30, 300, 25,$
% $\text{B3} = 10, 650, 50, \quad \text{B4} = 15, 200, 15$
     \\ \hline
    \end{tabular}
    \label{tab:constraints}
\end{table}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Comparison with Brute Force} \label{subsec: cpmare with brute force}
% %\SLI{Consolidating all the evaluation results into a single section may become overwhelming. Instead, we can divide them into multiple sections: one for the performance evaluation of our methods, one that highlights the key factors influencing our method's performance, and a third for comparing our performance to that of \gls{erica}.}

% In this section, we compare the brute-force (BF) method with our proposed techniques, \gls{algff} and \gls{algrp}. In all experiments, we use green for BF, shades of blue for \gls{algff}, and shades of red for \gls{algrp}. We evaluate the performance of these techniques using the \gls{dshealth} dataset with queries Q1 and Q2, as well as constraint C1 with different bounds using our default settings: a dataset size of 50K, 5 branches, top-7 solutions, and a bucket size of 15.

% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}[t]{1\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{comparison_fully_vs_ranges_bruteforce_Time.pdf}
%         \caption{Comparison of Runtime.}
%         \label{fig:runtime_comparison}
%     \end{subfigure}
%     \vspace{0.2cm} % Adjust vertical spacing if needed
%     \begin{subfigure}[t]{1\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{comparison_fully_vs_ranges_bruteforce_Checked Num.pdf}
%         \caption{Comparison of the number of Candidate solutions evaluated.}
%         \label{fig:checked_comparison}
%     \end{subfigure}
%     \vspace{0.2cm} % Adjust vertical spacing if needed
%     \begin{subfigure}[t]{1\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{comparison_fully_vs_ranges_bruteforce_Access Num.pdf}
%         \caption{Comparision of number of clusters accessed.}
%         \label{fig:access_comparison}
%     \end{subfigure}
%     \caption{Comparison of runtime, number candidate solutions evaluated, and number of clusters accessed for \gls{dshealth} dataset.}
%     \label{fig:comparison_combined}
%     \SLI{Shorten y-axis label, e.g., Number of Candidate Solutions Checked to NCSC, and increase the font size of y-axis.}
% \end{figure}


% \mypar{Performance}
% Figure~\ref{fig:runtime_comparison} illustrates the runtime of the three algorithms \textbf{BF, \gls{algff}, and \gls{algrp}} for queries Q1 and Q2 across constraint C1 with different bounds.
% % \SLI{What are the constraints from C1 to C6? What are the meaning of them? Eventually, the constraints in Table 3 should be explained.}
% The BF algorithm consistently exhibits the highest runtime, as it processes all data points for each repair and exhaustively evaluates all combinations, leading to significant computational overhead. Consequently, as shown in Figure~\ref{fig:access_comparison}, BF also incurs the highest number of accesses, as it scans every individual data point in the dataset. The \gls{algff} algorithm substantially reduces runtime by employing an optimized traversal technique that filters data based on the bounds of the clustering tree. Instead of accessing each data point, \gls{algff} only accesses cluster boundaries, as demonstrated in Figure~\ref{fig:access_comparison}, where it reduces the number of accesses. The \gls{algrp} algorithm further improves performance by efficiently pruning irrelevant repair combinations using range-based constraints. As observed in Figure~\ref{fig:access_comparison}, \gls{algrp} significantly minimizes the number of accesses to clusters, making it the most efficient approach.
% %For instance, under constraint C1B5, the runtime of the BF algorithm exceeds 38,000 seconds, whereas \gls{algff} and \gls{algrp} complete execution in approximately 2,900 seconds and 620 seconds, respectively. This result highlights that
% In general, \gls{algff} outperforms BF by at least an order of magnitude, while \gls{algrp} achieves an additional fivefold improvement, showcasing the efficiency of the proposed approaches.

% \mypar{Number of Candidate Solutions Checked}
% Figure~\ref{fig:checked_comparison} illustrates the number of candidate solutions evaluated by each algorithm for query Q1 and Q2 across different bounds of C1. The BF and \gls{algff} methods exhibit identical counts, as both exhaustively examine all possible repairs. In contrast, the \gls{algrp} method achieves the lowest number due to its efficient use of ranges. For example, under constraint C1B5, the BF and \gls{algff} methods evaluate over 7,400 constraints, as they individually assess each possible candidate repair. Meanwhile, the \gls{algrp} method evaluates approximately 850 candidate repair by leveraging ranges to skip sets of unpromising repairs. This reduction highlights the efficiency of the \gls{algrp} technique in eliminating redundant evaluations and minimizing computational overhead.
% Based on the results of the experiment, it is clear that the BF algorithm performs considerably worse than our proposed algorithms in terms of runtime. Given its poor performance and impracticality for real-world use cases, we have decided to exclude the BF algorithm from the remaining experiments. Instead, we will focus on comparing the \gls{algff} and \gls{algrp} algorithms, as they represent more realistic and competitive solutions.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htbp]
    \centering
    \begin{minipage}{1\linewidth}
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 30 0 0]{comparison_fully_vs_ranges_time_Healthcare.pdf}
        \caption{Runtime (sec) - \gls{dshealth} dataset.}
        \label{fig:ful_range_runtime_comparison_healthcare}
    \end{subfigure}
    % \vspace{-3mm}
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 30 0 0]{comparison_fully_vs_ranges_Time_ACSIncome.pdf}
        \caption{Runtime (sec) - \gls{dsacs} dataset.}
        \label{fig:ful_range_runtime_comparison_ACSIncome}
    \end{subfigure}
    \vspace{-3mm}
    \end{minipage}\\
    \begin{minipage}{1\linewidth}
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 30 0 0]{comparison_fully_vs_ranges_Checked Num_Healthcare.pdf}
        \caption{Total number of constraints evaluated (NCE) - \gls{dshealth} dataset.}
        \label{fig:ful_range_checked_comparison_healthcare}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 30 0 0]{comparison_fully_vs_ranges_Checked Num_ACSIncome.pdf}
        \caption{Total number of constraints evaluated (NCE) - \gls{dsacs} dataset.}
        \label{fig:ful_range_checked_comparison_ACSIncome}
    \end{subfigure}
    \vspace{-3mm}
    \end{minipage}\\
    \begin{minipage}{1\linewidth}
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 30 0 0]{comparison_fully_vs_ranges_Access Num_Healthcare.pdf}
        \caption{Total number of cluster accessed (NCA) - \gls{dshealth} dataset.}
        \label{fig:ful_range_access_comparison_healthcare}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 30 0 0]{comparison_fully_vs_ranges_Access Num_ACSIncome.pdf}
        \caption{Total number of cluster accessed (NCA) - \gls{dsacs} dataset.}
        \label{fig:ful_range_access_comparison_ACSIncome}
    \end{subfigure}
    \end{minipage}
    \vspace{-4mm}
    \caption{
    Runtime, \gls{NCE}, and \gls{NCA} for \gls{algff} and \gls{algrp} over the \gls{dshealth} and \gls{dsacs} datasets using the queries from~\Cref{tab:queries}.
    % Runtime, candidate solutions checked and number of clusters accesses comparison of our proposed algorithms.
    }
    \label{fig:checked_comparison_proposed}
     %\SLI{Fig 1(b): make the range on y-axis consistent }\SAI{Done}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Comparison of Proposed Techniques}
\subsection{Performance of \glsfmtshort{algff} and \glsfmtshort{algrp}}
\label{subsec: compare proposed techniques}
% In this section, we compare our proposed techniques \gls{algff} and \gls{algrp}.
We conduct experiments to measure the performance of \gls{algff} and \gls{algrp} using the \gls{dshealth} and \gls{dsacs} datasets with queries in~\Cref{tab:queries}, constraints in~\Cref{tab:constraints},
and default settings in~\Cref{sec:setup}.
For the \gls{dshealth}, the constraints $\propconstr_{1}$ and $\propconstr_{2}$ are used while $\propconstr_{3}$ and $\propconstr_{4}$ are considered for the \gls{dsacs}. In addition to runtime, we also measure \glsfmtfull{NCE} which is the total of number of repair candidates for which we evaluate the \gls{AC} and \glsfmtfull{NCA} which is the total number of clusters accessed by an algorithm.
% different queries and constraints with different boundaries
%using our
% The default setting for the parameters is as follows: a dataset size of 50K, 5 branches, 7 top solutions and a bucket size of 15.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Comparison with Brute Force}
We first compare our proposed methods, \gls{algff} and \gls{algrp}, with the \gls{algbf} method using the \gls{dshealth},
% along with
queries $Q_1$ and $Q_2$, and the constraint $\propconstr_{1}$.
As expected, both \gls{algff} and \gls{algrp} outperform \gls{algbf} by at least one order of magnitude in terms of runtime.
The \gls{algrp} algorithm significantly reduces both the total \gls{NCE} and the \gls{NCA}, while the \gls{algff} method maintains the same \gls{NCE} as \gls{algbf} but decreases the \gls{NCA} compared to \gls{algbf} (as \gls{algbf} does not use clusters we count the number of tuple accesses).
We present additional results in~\cite{AG25techrepo}.
% \SLI{Cite the extended version of the paper}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Runtime}
\label{par:Run Time}
% The performance comparison
% The runtime of our proposed \gls{algff} and \gls{algrp} techniques reveals consistent trends across datasets.
\Cref{fig:ful_range_runtime_comparison_healthcare,fig:ful_range_runtime_comparison_ACSIncome} show the runtime of the \gls{algff} and \gls{algrp} algorithms for \gls{dshealth} and \gls{dsacs}, respectively.
For given constraint $\propconstr_i$ we vary the bounds $[B_l,B_u]$ to control what percentage of repair candidates have to be processed by \gls{algbf} and \gls{algff} to determine the top-$k$ repairs as explained above. For example, $\propconstr_{1}^{d=38}$ in~\Cref{fig:ful_range_runtime_comparison_healthcare} for $Q_1$ is the constraint $\propconstr_{1}$ from~\Cref{tab:constraints} with the bounds set such that 38\% of the candidate solutions have to be explored by these algorithms. We refer to this as the \gls{ED}.
% The x-axis shows pairs of a constraint used and the proximity of solutions (exploration distance)
% % The exploration distance
% which is defined as the ratio of
% the actual number of candidate solutions checked by the algorithm for the given top-$k$ to the total number of candidate solutions available.
% For example, $\propconstr_{1}^{d=38}$ in~\Cref{fig:ful_range_runtime_comparison_healthcare} for $Q_1$ presents the constraint $\propconstr_{1}$ in~\Cref{tab:constraints} with a bound
% where solutions can be found after exploring $38\%$ of the search space.
% The y-axis shows the execution time of our methods.
 \gls{algrp} (pink bars) generally outperforms \gls{algff} (blue bars) for most settings.
% However, in the \gls{dsacs} dataset,
% (Figure~\ref{fig:ful_range_runtime_comparison_ACSIncome}),
In~\Cref{fig:ful_range_runtime_comparison_ACSIncome}, two algorithms exhibit similar performance for
% constraints C3B4 and C3B5 in
$Q_4$ with $\propconstr_{3}$, where solutions are found after exploring only 2\% and 3\% of the search space.
% , respectively.
A similar pattern is observed
%for C3B6
 for $Q_5$ with $\propconstr_{3}^{d=3}$ and $Q_6$ with $\propconstr_{4}^{d=4}$.
We further investigate the relationship between %the exploration distance 
the \gls{ED} and the runtime of our algorithms in~\Cref{subsec: invistigation}.
% , where the solution is located after 3\% of the search space.
% In contrast, for constraints such as C3B1, C3B2, C3B7, and C3B8,
In general, \gls{algrp} significantly outperforms \gls{algff}, demonstrating an improvement of about an order of magnitude due to its capability of pruning and confirming sets of candidate repairs at once.
% This performance gain is attributed to \gls{algrp}'s ability to efficiently explore the search space by leveraging range-based pruning rather than exhaustively evaluating all possible candidates.
% A key insight from these findings is that the efficiency of \gls{algrp} is strongly influenced by the proximity of solutions within the search space. When solutions are closer to the start,
% \gls{algff} quickly locates the answer.
%fewer explorations are required, allowing \gls{algff} to quickly locate the answer. Conversely, \gls{algrp} needs to examine multiple ranges, leading to increased %execution
% runtime.
% This observation explains the comparative performance of \gls{algrp} and aligns with the observed trends.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Total \glsfmtfull{NCE}}
We further analyze how \gls{NCE} affects the performance of our methods.
\Cref{fig:ful_range_checked_comparison_healthcare,fig:ful_range_checked_comparison_ACSIncome} shows the result of the \gls{NCE} (on the y axis) for \gls{algff} and \gls{algrp} on \gls{dshealth} and \gls{dsacs}, respectively.
\Gls{algrp} consistently checks fewer candidates compared to \gls{algff}.
% which evaluates each possible repair individually.
% , while \gls{algrp} efficiently reduces the number of evaluations through the range-based pruning algorithm (\Cref{subsec: optimized gorithm}).
% However, as shown in \gls{dsacs}
% % , constraints C3B4 and C3B5 in
% for $Q_4$,
% show comparable performance between \gls{algff} and \gls{algrp}, reinforcing the earlier observation that
As observed in the runtime evaluation, the \gls{ED} impacts the efficiency of our algorithms, producing comparable results for \gls{algff} and \gls{algrp} when a small number of candidates has to be explored, e.g., as shown in~\Cref{fig:ful_range_checked_comparison_ACSIncome} for $Q_4$ with $\propconstr_{3}^{d=2}$ and $Q_5$ with $\propconstr_{3}^{d=3}$.
% Similarly, this inversion is observed in the result of $Q_5$,
% % An inversion is observed in $Q_5$ for constraint C3B6, where \gls{algff} performs 592 checks compared to 809 by \gls{algrp},
% further highlighting the impact of %exploration distance
% proximity on performance.
% The impact of solution proximity is further supported by the analysis of the number of candidate solutions checked.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Total Number of Cluster Accessed (NCA)}
% A similar trend is observed in
The results of the number of clusters accessed are shown in ~\Cref{fig:ful_range_access_comparison_healthcare,fig:ful_range_access_comparison_ACSIncome} for \gls{dshealth} and \gls{dsacs}, respectively. Similarly, \gls{algrp} accesses significantly fewer clusters than \gls{algff}, highlighting its efficiency in limiting the exploration of the search space. Furthermore, it follows the same trend of the previous evaluation results such that the benefit of \gls{algrp} becomes negligible and may even reverse when the proximity of solutions is low.

% In the \gls{dshealth} dataset, \gls{algrp} generally accesses fewer clusters than \gls{algff}, demonstrating its efficiency in limiting search space exploration. However, in the \gls{dsacs} dataset (Figure~\ref{fig:ful_range_access_comparison_ACSIncome}), the differences are more nuanced. For constraints C3B4 and C3B5 in Q4, both techniques access a similar number of clusters. In contrast, for C3B6 in Q5, \gls{algrp} accesses more clusters (809) compared to \gls{algff} (592). This reflects a scenario where \gls{algrp}’s clustering mechanism required exploring a greater portion of the search space when solutions were positioned closer to the beginning. As a result, \gls{algrp} lost some of its efficiency compared to \gls{algff} in these specific cases.
% However, for constraints C3B1, C3B2, C3B7, and C3B8, \gls{algrp} accesses fewer clusters, as shown in Figure~\ref{fig:ful_range_access_comparison_ACSIncome}, by exploiting range-based pruning. Additionally, \gls{algrp} evaluates fewer candidate solutions, as illustrated in Figure~\ref{fig:ful_range_checked_comparison_ACSIncome}. This confirms that \gls{algrp} is highly effective when solutions are distant but may lose its advantage when solutions are found early in the search process.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{%Evaluation of
Performance-Impacting Factors}
\label{subsec: invistigation}

To gain deeper insights into the behavior observed in~\Cref{subsec: compare proposed techniques}, we  investigate the relationship between the \glsfmtfull{ED} and performance.
% in Section~\ref{subsec: invistigation}.
% This analysis will provide valuable guidance for refining query optimization techniques in real-world applications.
%
% In this section, we compare the performance of our proposed techniques, \gls{algff} and \gls{algrp}, in relation to exploration distance.
% The exploration distance is defined as the ratio of
% the actual number of candidate solutions checked by the algorithm for the given Top-$k$
% to the total number of candidate solutions available.
Additionally, we evaluate the performance of \gls{algff} and \gls{algrp} in terms of the parameters
% , bucket size and branching factor
from~\Cref{sec:setup}.
%We evaluate the performance of these techniques using
We use the \gls{dshealth}, \gls{dsacs}, and \gls{tpch} datasets.
% and default settings in~\Cref{sec:setup}.
% , considering different queries and constraints with varying boundaries using our default settings: a dataset size of 50K, 5 branches, 7 top solutions and a bucket size of 15.

%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering \vspace{-8mm}
    % First row
    \begin{subfigure}[t]{0.98\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Time_vs_constraint_distance_combined_Healthcare.pdf}
        % \caption{\gls{dshealth} dataset.}
        % \label{fig:distance_runtime_comparison_healthcare}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}[t]{0.49\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{Time_vs_constraint_distance_combined_ACSIncome.pdf}
    %     \caption{\gls{dsacs} dataset.}
    %     \label{fig:distance_runtime_comparison_ACSIncome}
    % \end{subfigure}
    \vspace{-2mm}
    % Overall caption for the figure
    \caption{Runtime of \gls{algff} and \gls{algrp}, varying \gls{ED}.
    % using the \gls{dshealth} dataset
    % comparison of our proposed algorithms.
    }
    % \SLI{Range y-axis from 10 to the 1}
    \label{fig:healthcare-proximity}
\end{figure}
%%%%%%%%%%%%%%%

% \subsubsection{Effect of Solution Exploration Distance}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Effect of \Glsfmtlong{ED}}
%
\captionsetup[figure]{skip=5pt} % Adjust the value as needed
% \SLI{Overlaps with the results in Sec 6.2. Should we explain the exploration distance here? Or, Should we keep it in Sec 6.2 and remove it from here?}
% \SAI{I consider what we found in 6.2 is leading us to do the investigation in 6.3}
We
% focus on a deeper investigation by
use queries $Q_1$–$Q_3$ and the constraint $\propconstr_{1}$ on \gls{dshealth}  and vary the bounds to control for \gls{ED}.
The result is shown in~\Cref{fig:healthcare-proximity}.
We present results for \gls{dsacs} in~\cite{AG25techrepo}.
% \SLI{cite the extended version}
For $Q_1$ and $Q_2$, when \gls{ED} $10\%$ or less, \gls{algff} and \gls{algrp} exhibit comparable performance.
A similar pattern is seen for $Q_3$, where \gls{algff} performs better than \gls{algrp} for lower \gls{ED}, but \gls{algrp} outperforms \gls{algff} for \gls{ED} $> 50\%$.
% For $Q_3$, \gls{algrp} starts to outperform around $50\%$ because...
% \SLI{Can we reason about this?}
% \SAI{Here because as you see we don't have points between 10-50 as the chosen random bounds don't generate distance between 10-50 for Q3. so I feel we can say in general that Q3 confirms that as far as we get the distance, \gls{algrp} outperform}
The reason behind these trends is that when solutions are closed to the user query (smaller \gls{ED}), then there is a lower chance that \gls{algrp} can prune larger sets of candidates at once.

% In general, as \gls{ED} increases, %we observe
% the performance gap widens,
% % indicating that the \gls{algrp} becomes increasingly efficient compared to \gls{algff}.
% a clear advantage of \gls{algrp}.
% As highlighted in \Cref{subsec: compare proposed techniques}, constraints with solutions located farther in the search space favor \gls{algrp}, while those closer to the beginning may reduce its advantage.
% The reason behind these trends is that when solutions are closer to the start of the search space, \gls{algff} requires fewer explorations, allowing it to quickly locate a solution that satisfies the constraint. Conversely, \gls{algrp} must examine multiple ranges from the beginning of the search space, leading to increased execution time.


% We investigate the impact of solution distance on our proposed algorithms by running queries $Q_1$–$Q_3$ with constraint $\propconstr_{1}$ on the \gls{dshealth} dataset using different bounds, and queries $Q_4$–$Q_6$ with constraint $\propconstr_{1}$ on the \gls{dsacs} dataset under varying bounds.

% In the \gls{dshealth} dataset, we observe same trends across all three measures (Runtime, Candidate solutions checked and Clusters accessed) as Figure \ref{fig:distance_runtime_comparison_healthcare}; therefore, we do not present them here. For Query 1, when the distance is approximately 10\% and less, \gls{algff} and \gls{algrp} exhibit comparable performance. Similarly, in Queries 2 and 3, when the distance is between 0\% and 3\%, both algorithms perform similarly. However, as the distance increases, we observe a clear advantage for \gls{algrp}, the performance gap widens, indicating that the \gls{algrp} becomes increasingly efficient compared to Fully Filtering Repair. This confirms our previous claim that the \gls{algrp} benefits more when solutions are located farther in the search space.

% Similarly, in the ACSIncome dataset, the trends across all three measures as Figure \ref{fig:distance_runtime_comparison_ACSIncome}. For Queries 4 and 5, when the distance is less than 10\%, \gls{algff} consistently outperforms \gls{algrp}. However, as the distance surpasses 10\%, the performance dynamics shift, favoring \gls{algrp}. This change is reflected by a noticeable reduction in the number of clusters accessed and a decrease in runtime, illustrating that \gls{algrp} becomes increasingly effective as the search space expands.

% The reason behind these trends is that when solutions are closer to the start of the search space, \gls{algff} requires fewer explorations, allowing it to quickly locate a solution that satisfies the constraint. Conversely, \gls{algrp} must examine multiple ranges from the beginning of the search space, leading to increased execution time. These observations reinforce the assertion that the efficiency of the \gls{algrp} repair technique improves as the exploration distance increases, while \gls{algff} maintains an advantage in scenarios where solutions are in closer proximity.

%\SLI{Add justification why range-based repair works better as distance increases.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[H]
%     \centering \small
%     \begin{tabular}{|c|c|c|}
%         \hline
%         \textbf{No. of Branches} & \textbf{No. of Leaf Clusters} & \textbf{No. of Data Points} \\
%         \hline
%         5  & 15625  & 3 or 4  \\
%         10 & 10000  & 10      \\
%         15 & 3375   & 14 or 15 \\
%         20 & 8000   & 6 or 7  \\
%         25 & 15625  & 3 or 4  \\
%         30 & 27000  & 1 or 2  \\
%         \hline
%     \end{tabular}
%     \vspace{-2mm}
%     \caption{Branching Configuration and Data Distribution}
%     \SLI{Is the number of data points for each node?}
%     \label{tab:branching_data}
% \end{table}


%%%%%%%%%%%%%
\begin{figure}[t]
    \centering \vspace{-6.5mm}
    % First set of subfigures
    \begin{subfigure}[t]{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 40 0 0]{comparison_fully_vs_ranges_Time_Healthcare_BucketSize.pdf}
        \caption{\gls{dshealth} dataset}
        \label{fig:BucketSize_Time_Healthcare}
    \end{subfigure}
    \vspace{-3mm}
    \begin{subfigure}[t]{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 40 0 0]{comparison_fully_vs_ranges_Time_ACSIncome_BucketSize.pdf}
        \caption{\gls{dsacs} dataset}
        \label{fig:BucketSize_Time_ACSIncome}
    \end{subfigure}
    \vspace{-1mm}
    % Overall caption for the figure
    \caption{Runtime, varying bucket size \bucketsize.
    % comparison of our proposed algorithms
    % for different bucket sizes.
    % (a) \gls{dsacs} dataset. (b) \gls{dshealth} dataset.
    }
    \label{fig:BucketSize_comparison}
  \end{figure}

%%%%%%%%%%%%%%%%%%%%%
\mypar{Effect %of Number
of Bucket Size}
\label{subsub: effect of bucketSize}
%
We now evaluate the runtime of \gls{algff} and \gls{algrp} varying the bucket size \bucketsize using $Q_1$ with $\propconstr_{1}$ using bounds $[0.44, 0.5]$ for the \gls{dshealth} dataset and $Q_4$ with $\propconstr_{3}$ using bounds $[0.34, 0.39]$ for the \gls{dsacs} dataset.
% The same queries, constraints, and datasets in the previous evaluation are used here.
% In this section, we evaluate the \gls{dsacs} and \gls{dshealth} datasets by employing Query Q1 with C1 for \gls{dshealth} and Q4 with C3 for \gls{dsacs}, as listed in Table \ref{tab:queries} and Table \ref{tab:constraints}.
% While data size is set to 50K, branch size is at 5, and top-$k$ = 7,
We vary the \bucketsize from 5 to 2500.
% Selecting different size of buckets results in varying the number of leaf clusters and data points in each leaf.
% to highlight their impact on performance.
% \SLI{Should be moved to earlier: \\
Using the default branching factor \branchfactor of 5,
%an example
the structure of the \tree for this evaluation is
% remains fixed across different bucket branches
as follows:
(i) Level 1: 5 clusters, each with 10,000 data points;
(ii) Level 2: 25 clusters, each with 2,000 data points;
(iii) Level 3: 125 clusters, each with 400 data points;
(iv) Level 4: 525 clusters, each with 80 data points;
(v) Level 5: 3,125 clusters, each with 16 data points;
(vi) Level 6: 15,625 clusters, each with 3 or 4 data points.
% }
Note that the algorithms will generate \tree up to the level where the capacity of each cluster at that level is less than or equal to \bucketsize.
For example, for $\bucketsize= 200$, the tree will have 4 levels.
%
% The only variation across different bucket sizes lies in determining at which level the algorithm stops exploring further. As discussed in Section \ref{subsub:Effect of branches}, both the \gls{algff} and \gls{algrp} algorithms are influenced by the number of clusters at the leaf level, where an increase in the number of leaf clusters leads to higher runtime. Additionally,
The results of this experiment are shown in~\Cref{fig:BucketSize_comparison}. The advantage of smaller bucket sizes is that it is more likely that we can find a cluster that is fully covered / not covered at all. However, this comes at the cost of having to explore more clusters. In preliminary experiments, we have identified $\bucketsize=15$ to yield robust performance for a wide variety of settings and use this as the default.

% For the \gls{algff} algorithm, when the bucket size is 5, the algorithm leads to the worst performance for \gls{algff} where it traverses the largest number of leaves (15,625). For the smaller bucket size (up to bucket size $\simeq$ 200), the runtime decreases as the bucket size increases. Upon the bucket size becoming larger, e.g., 1000 and 2000, the runtime increases. Although the algorithms check a smaller number of clusters in the \tree, each cluster contains many data points, which reduces filtering opportunities. A similar trend can be seen in the results of \gls{dsacs}.
% The results of the \gls{algrp} algorithm also align with this trend. \gls{algrp} tends to perform better with smaller bucket sizes because it can effectively prune more buckets. When the buckets are small, each leaf may contain only 3 or 4 data points, which reduces the need for further searching. However, as shown in~\Cref{fig:BucketSize_Time_ACSIncome}, the performance of \gls{algrp} may decline compared to \gls{algff} when the bucket size is large. Larger buckets contain more data points, which diminishes the filtering advantages of \gls{algrp}.
% a mix of solutions and non-solutions, requiring further subdivision and increasing computational complexity.

% \gls{algrp} is particularly affected by the number of data points within each cluster at the leaf level. When leaf clusters contain more data points, \gls{algrp} struggles to efficiently identify solutions, as larger buckets contain a mix of solutions and non-solutions, requiring further subdivision and increasing computational complexity.

% As shown in Figure \ref{fig:BucketSize_comparison}, across both datasets, when the bucket size is 5, the algorithm stops at level 6, where the number of leaf clusters is at its maximum (15,625), leading to the worst performance for \gls{algff}. This supports our claim that \gls{algff}'s runtime increases with the number of leaf clusters. On the other hand, \gls{algrp} performs best in this scenario, as it benefits from pruning smaller buckets, where each leaf cluster contains only 3 or 4 data points, eliminating the need for further subdivision. However, for bucket sizes of 1,000 and 2,500, the algorithm stops at levels 2 and 3, respectively. In these cases, the larger number of data points per leaf cluster (2,000 and 400, respectively) makes it difficult for \gls{algrp} to efficiently include or exclude clusters, leading to additional exploration and increased runtime.

% For the \gls{dsacs} dataset, as shown in Figure \ref{fig:BucketSize_Time_ACSIncome}, when the bucket size is 2,500, \gls{algrp} performs worse than \gls{algff}, as it struggles to find the solution due to excessive subdivision. In contrast, for the \gls{dshealth} dataset, as seen in Figure \ref{fig:BucketSize_Time_Healthcare}, \gls{algrp} still outperforms \gls{algff} at a bucket size of 2,500, but it exhibits the worst runtime compared to other bucket sizes.


\begin{table}[H]
    \centering
    \vspace{-1mm}
    \caption{Branching Configuration and Data Distribution}
    \vspace{-2mm}
    \begin{tabular}{|c|c||c|c|}
        \hline
        \textbf{\# of Branches} & \textbf{\# of Leaves} & \textbf{\# of Branches} & \textbf{\# of Leaves} \\
        \hline
        5  & 15625  & 20 & 8000 \\
        10 & 10000  & 25 & 15625   \\
        15 & 3375   & 30 & 27000 \\
        \hline
    \end{tabular}
    % \SLI{Clustering tree for which dataset?}
    % \SAI{This will be for both dataset since we have the same default setting (50K data size, 15 bucket size, so for each branch we have the same structure for both dataset}
    \label{tab:branching_data}
    % \SLI{@Shatha: can you add more information about the tree structure? For example, how the depth of the cluster tree changes? Why is the number of leaf clusters similar in (5,25) and (10,20)?} \SAI{Here each branch factor creates different depth, so with (5 branches> 6 levels), (10 branches> 4 levels), and (15, 20, 25 30 > 3 levels). It appears that the performance doesn't affected by the depth of the tree only of by how many clusters node at the leaf level. I am not sure if we have to add the depth to the table. For similar number of leaf clusters, if we divide the 50k into 15 buckets and the number of given branches, it will give us these numbers of leaves.}
\end{table}

\begin{figure}[t]
    \centering 
    \vspace{-3mm}
    % First set of subfigures
    \begin{subfigure}[t]{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 30 0 0]{comparison_fully_vs_ranges_Time_Healthcare_BranchNum.pdf}
        \caption{\gls{dshealth} dataset}
        \label{fig:BranchNum_Time_ACSIncome_Healthcare}
    \end{subfigure}
    \begin{subfigure}[t]{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 30 0 0]{comparison_fully_vs_ranges_Time_ACSIncome_BranchNum.pdf}
        \caption{\gls{dsacs} dataset}
        \label{fig:BranchNum_Time_ACSIncome}
    \end{subfigure}
    % \SLI{Increase the font size of labels}
    % \SAI{Updated in all figures}
    \vspace{-3.5mm}
    % Overall caption for the figure
    \caption{
    Runtime, varying the number of branches \branchfactor.
    % Time comparison of our proposed algorithms for different numbers of branches. (a) \gls{dsacs} dataset. (b) \gls{dshealth} dataset.
    }
    \label{fig:num-of-branch-perf}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Effect of the Branching Factor} \label{subsub:Effect of branches}
%
We now examines the relationship between the branching factor \branchfactor and the runtime of the \gls{algff} and \gls{algrp}. 
% algorithms.
% , using $Q_1$ with $\propconstr_{1}$ for the \gls{dshealth} dataset and $Q_4$ with $\propconstr_{3}$ for the \gls{dsacs} dataset.
We use the same queries, constraints, bounds, and datasets as in the previous evaluation.
In this experiment, we vary the \branchfactor from 5 to 30. The corresponding number of leaf nodes in the \tree is shown in~\Cref{tab:branching_data}.
As we use the default bucket size $\bucketsize = 15$, the branching factor affects the depth of the tree.
% While varying the number of branches, the depth of the \tree changes as each cluster at the parent level needs to be split until it reaches the desired bucket size which is default = 15 in this case.
% For example, 5 branches produces a cluster of depth of 6 whereas 30 branches yields a cluster of depth of 3.
% Interestingly, for each number of branches, the structure of the clusters remains the same across both datasets.
% , as the data size and bucket size are fixed at 50K and 15, respectively.
The result shown in~\Cref{fig:num-of-branch-perf} confirms that the performance of \gls{algff} and \gls{algrp} correlates with the number of clusters at the leaf level. For the \gls{algff}, %algorithm, 
the branching factors of 5 and 25 yield nearly identical runtime because both have the same number of leaves (15,625). A similar pattern can be observed for $\branchfactor=10$ and $\branchfactor=20$. At $\branchfactor=15$, \gls{algff} achieves the lowest runtime, as it involves the smallest number of leaves (3,375). For $\branchfactor=30$, the number of leaf clusters significantly increases, leading to a substantial rise in the runtime of \gls{algff}.
These results also demonstrate that the tree depths only has negligible impact on the runtime.
% % We claim that
% the performance of \gls{algff} and \gls{algrp} follows the trend of the number of clusters at the leaf level.
% % is affected by the number of clusters at the leaf level.
% % Table \ref{tab:branching_data} clearly shows the structure of the clustering tree at leaf level for each branch. In figure \ref{fig:BranchNum_comparison}
% For \gls{algff} over the two datasets, the branching factors of 5 and 25 exhibit nearly consistent runtime as both have the same number of leaf clusters (15,625). A similar trend is observed for branching factors of 10 and 20.
% % for both datasets.
% % However,
% At the branching factor of 15, \gls{algff} achieves the lowest runtime
% %due to its reduced
% as the lowest number of leaf clusters (3,375) is involved.
% The number of leaf clusters jumps at the branching factor of 30 where the runtime of \gls{algff} also substantially increases.
% % Conversely, when the number of branches increases to 30, the algorithm experiences its worst performance, with a significant increase in the number of clusters accessed, as the number of leaf nodes rises substantially.
% % For \gls{algrp}, the algorithm performs similarly to \gls{algff},
For \gls{algrp}, overall performance trends align with those of \gls{algff}.
However, \gls{algrp} is less influenced by the branching factor. % As a comparison between the two algorithms, \gls{algrp} consistently outperforms \gls{algff}, demonstrating greater efficiency across the datasets.
% in managing search complexity.
% Other measurements exhibit the same trend; therefore, we do not present them here.

%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \vspace{-3mm}
    % First set of subfigures
    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 40 0 0]{comparison_fully_vs_ranges_Time_ACSIncome_TopK.pdf}
        \caption{Runtime(sec)\newline}
        \label{fig:topk_Time}
    \end{subfigure}
    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 40 0 0]{comparison_fully_vs_ranges_Checked Num_ACSIncome_TopK.pdf}
        \caption{Number of constraints evaluated }
        \label{fig:topk_NCE}
    \end{subfigure}
    %5\begin{subfigure}{0.45\linewidth}
        %\centering
        %\includegraphics[width=\linewidth, trim=0 20 0 0]%{comparison_fully_vs_ranges_Access Num_ACSIncome_TopK.pdf}
    %\end{subfigure}
    % Overall caption for the figure
    \vspace{-3.5mm}
    \caption{Performance of \gls{algff} and \gls{algrp} over top-$k$
    % and Runtime Comparison of our proposed algorithms.
    }
    \label{fig:TopK_comparison}
\end{figure}
%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Effect of $k$}
\label{subsub: effect of top-k}
In this experiment, we vary the parameter $k$ from 1 to 15.
% as 1 is a single solution.
% The total number of candidate solutions exist is 17664. As the Top-K value
For both \gls{algff} and \gls{algrp}, as $k$ increases, the runtime also increases, as shown in~\Cref{fig:topk_Time}.
This behavior is expected since finding a single repair ($k$=1) requires less computation than identifying multiple repairs. When $k$ is larger, the algorithm must explore a larger fraction of the search space to find additional repairs.
% , leading to time increase.
%\SLI{@Shatha: Do we have graphs for the below paragraph? If not, please make the graph in Figure 5 wider and shorter in height.}\SAI{I have the other figures, I added them, but because they follow the same trend as runtime, I did not present them, now I present only NCE figure}
Similarly, both the \gls{NCE} as shown in~\Cref{fig:topk_NCE} and \gls{NCA} exhibit the same increasing trend. This pattern is observed consistently across both \gls{algff} and \gls{algrp}, reinforcing the intuition that retrieving more solutions requires higher computational effort. % Overall, across different top-$k$ values,
 \gls{algrp} consistently outperforms \gls{algff}.

%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering 
    \vspace{-3mm}
    % First set of subfigures
    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 40 0 0]{comparison_fully_vs_ranges_Time_TPC-H_DataSize.pdf}
        \caption{Runtime (sec)}
        \label{fig:DataSize_Time}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 40 0 0]{comparison_fully_vs_ranges_Access Num_TPC-H_DataSize.pdf}
        \caption{Number of clusters accesses}
        \label{fig:DataSize_Clusters_Accesses}
    \end{subfigure}
    % Overall caption for the figure
    \vspace{-4mm}
    \caption{Evaluation result over TPC-H dataset
    % Comparison of our proposed algorithms for different data sizes of TPC-H. (a) Runtime. (b) Number of Clusters Accessed.
    }
    \label{fig:BranchNum_comparison}
\end{figure}
%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Effect of Dataset Size}
\label{subsub:Effect of data size}
% In this section, we vary the data size from 25K to 500K, analyzing its impact on algorithm performance.
%\SLI{What is the query, constraint, and parameters used?}
Next, we vary the dataset size and measure the runtime and the \gls{NCA} for the \gls{tpch} dataset, $Q_7$ from~\Cref{tab:queries}, $\propconstr_{5}$ from~\Cref{tab:constraints}. We use default settings for all parameters (\Cref{sec:setup}).
As shown in~\Cref{fig:DataSize_Time}, as the data size increases, the runtime also increases.
% This behavior is expected, as larger datasets require more computations to process and retrieve valid solutions.
Dataset size impacts both the size of the search space and the size of the kd-tree. Nonetheless, our algorithm scale roughly linearly in dataset size demonstrating the effectiveness of using materialized aggregation results for clusters and range-based pruning of candidate repair sets.
% While increasing data size,
% both \gls{algff} and \gls{algrp} must explore a larger search space. Furthermore, dataset size also affects the size of the clustering tree.
This is further supported by the \gls{NCA} measurements
% , leading to higher execution times.
% Similarly, NCA follows the same increasing trend, as shown in~\Cref{fig:DataSize_Clusters_Accesses}.
shown in~\Cref{fig:DataSize_Clusters_Accesses},
which exhibit the same trend as the runtime.
% which contributes to computational overhead.
% This pattern holds consistently across both \gls{algff} and \gls{algrp}, reinforcing the idea that processing larger datasets demands greater effort.
%
% Overall, across different dataset sizes, \gls{algrp} consistently outperforms \gls{algff}.
% , demonstrating superior efficiency in managing search complexity while reducing the number of clusters accessed and overall runtime.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Comparison with Related Work} \label{subsec: compare with related work}
%
We compare our approach with \gls{erica}~\cite{LM23}, which solves the related problem of finding all minimal refinements of a given query that satisfy a set of cardinality constraints
for groups within the result set. Such constraints are special cases on the \glspl{AC} we support.  \gls{erica} returns all repairs that are not \emph{dominated} by any other repair where a repair dominates another repair if it is at least as close to the user query for every condition $\theta_i$ and strictly closer in at least one condition.  That is, \gls{erica} returns the skyline~\cite{BK01b}. Thus, different from our approach, the number of returned repairs is not an input parameter in \gls{erica}. For a fair comparison, we determine the minimal repairs and then set $k$ such that our methods returns a superset of the repairs returned by \gls{erica}.
% cardinality constraints over groups in the query output by generating all minimal refinements. % To facilitate the comparison,
To conduct the evaluation for \gls{erica},
we used
% \gls{erica}'s datasets, queries, constraints, and
% . We used
the available Python implementation (\url{https://github.com/JinyangLi01/Query_refinement}).\footnote{We did modify the the code for a more fair comparison of algorithms regarding the evaluation of constraints as this part of our implementation is implemented in pure Python while \gls{erica} used Pandas Dataframe operations that are implemented in C. We leave a full implementation of our methods in a lower-level language such as C++ to future work.}
% provided by Li et al.~\cite{LM23}.
%
We adopt the queries, constraints, and the dataset from~\cite{LM23}.
We compare the generated refinements and runtime of our techniques with \gls{erica} using $Q_1$ and $Q_2$ (\Cref{tab:queries}) on the \gls{dshealth} dataset (size 50K) with constraints $\propconstrset_{6}$ and $\propconstrset_{7}$ (\Cref{tab:constraints}), respectively.
% \SAI{here I want to add that these datasets, queries and constraints are \gls{erica}'s queries and constraints}
% \SLI{It is also mentioned in Section 6.1.}


% \SAI{I want to add that B1 in C1B1 in figure7 and so on are different bounds for the constraints}
% \SLI{Are the bounds the same as in \gls{erica}?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Comparison on the Generated Repairs}
%
We first compare the generated repairs by our approach and \gls{erica}.
For $Q_1$ with $\propconstrset_{6}$, \gls{erica} generates 7 minimal repairs whereas our technique generates 356, including those produced by \gls{erica}. Similarly, for $Q_2$ with $\propconstrset_{7}$, \gls{erica} generates 9 minimal repairs while our approaches generates 1035, including those produced by \gls{erica}.
In general, our techniques successfully generates all repairs produced by \gls{erica}.
% \SLI{Do not understand the below sentence: \\
% None of the generated repairs by \gls{erica} were close to the user query as the repairs found by our approach.
% }
% \SAI{
% similar to the original user queries while \gls{erica} generates repairs that are far a way from the user query (for example if we have predicate Age>35, our approach trying to generate a similar repair like 34, 36, 37 ... and so on, while \gls{erica} generates a far repair like Age >70)
% }
Note that the top-1 repair returned by our approach is guaranteed to be minimal (not dominated by any other repair). However, the remaining minimal repairs returned by \gls{erica} may have a significantly higher distance to the user query than the remaining top-k answers returned by our approach.
% Note that our approaches generate repairs that are closer to the original user queries compared to the repairs by \gls{erica}.
For example, in $Q_2$, given the condition \texttt{num-children >= 4} of the user query, our solution includes a refined condition \texttt{num-children >= 3} whereas \gls{erica} provides a refinement \texttt{num-children >= 1} which is far from the user query.
% \SLI{Is the example based on an evaluation result?} \SAI{now it based on an evaluation result}
% The differences in the results arise from the definitions of minimality defined by the two approaches. \gls{erica} considers user preferences, focusing on repairs that best satisfy these preferences.
% In contrast, our approach emphasizes similarity to the original user query by exploring the space of actual values for each predicate.
As mentioned above, to ensure that our approach returns a superset of the solutions returned by \gls{erica}’s solutions, we did adjusted $k$ per query and constraint set to ensure that. % demonstrating that our technique encompasses \gls{erica}’s solutions while offering additional repairs.
% However, increasing the Top-$k$ parameter penalizes the runtime of our techniques.


%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.46\linewidth}
        \centering
        \includegraphics[width=\linewidth,trim=0 30 0 0]{Search_time_comparison.pdf}
        \caption{Pre-processing}
        \label{fig:Erica_SearchTime}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth,trim=0 30 0 0]{Prov_time_comparison.pdf}
        \caption{Search}
        \label{fig:Erica_ProvTime}
    \end{subfigure}
    \vspace{-3mm}
    \caption{Runtimes of \gls{algff}, \gls{algrp}, and \gls{erica}.}
    \label{fig:Eric_comparison}
\end{figure}
%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Runtime Comparison}
%
The experiment utilizes $Q_4$ with $\propconstrset_{8}$
%under different bounds
on the 50K \gls{dsacs} dataset, which is derived from \gls{erica}’s dataset, query, and constraint.
%\SLI{What is $k$ and what is the number of repairs by Erica?}\SAI{For constraints C8B1 and C8B2 (k=17), for C8B3 (k=11) and for C8B4 (k=13)}
We use the same bounds in the constraints for both \gls{erica} and our algorithms:
$B1 \defas (B_{u_1} = 30, B_{u_2} =150, B_{u_3} =10)$ and $B2 \defas (B_{u_1} =30,B_{u_2} =300,B_{u_3} =25)$, $B3 \defas (B_{u_1} =10, B_{u_2} =650, B_{u_3} =50)$, and $B4 \defas (B_{u_1} =15,B_{u_2} = 200, B_{u_3} =15)$.
To ensure a fair comparison of execution time, we fix the number of generated repairs (i.e., Top-$k$) in our approach to equal to the number of repairs produced by \gls{erica}. We set $k$=17 for constraintsets $\propconstrset_{8}^{B1}$ and $\propconstrset_{8}^{B2}$, $k$=11  for $\propconstrset_{8}^{B3}$,  and $k$=13 for $\propconstrset_{8}^{B4}$.
%\SLI{@Shatha: place the correct bounds here}
Due to the different optimization criterions, variations in the generated repairs between our approach and \gls{erica} are expected.
The results in~\Cref{fig:Erica_SearchTime} reveal an advantage of the \gls{algrp} algorithm, which outperforms \gls{erica} in search time which is the time of exploring the search space to generate a repair.
% This suggests that \gls{algrp} is more efficient in exploring the search space and identifying candidate repairs.
However, as shown in~\Cref{fig:Erica_ProvTime}, in pre-processing time which is the time of materializing aggregates and constructing the kd-tree for our methods and generating provenance expressions for \gls{erica}, \gls{erica} outperforms both \gls{algrp} and \gls{algff}, indicating that \gls{erica} summarizes information needed for the search process more effectively. Overall the total runtime of \gls{algrp} and \gls{erica} are comparable, even through our approach does not apply any specialized optimizations that exploit the monotonicity of the constraints supported in \gls{erica}, while our approach supports a significantly broader class of constraints that include common fairness notions such as \gls{SPD}.
These results also highlight the need for our range-based optimizations in \gls{algrp}, as \gls{algff} is significantly slower than \gls{erica}.
% both search and provenance times, reinforcing the efficiency benefits of \gls{algrp} technique.
% While \gls{erica} demonstrates faster pre-processing computation, our \gls{algrp} technique excels in efficiently handling more challenging constraints, providing broader applicability compared to \gls{erica}~\cite{LM23}.


%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "../main"
%%% End:

